Refactoring to Pythonic Idioms: A Hybrid Knowledge-Driven Approach Leveraging Large Language Models

Pythonic idioms are highly valued and widely used in the Python programming community. However, many Python users find it challenging to use Pythonic idioms. Adopting a rule-based approach or LLM-only approach is not sufficient to overcome three persistent challenges of code idiomatization including code miss, wrong detection and wrong refactoring. Motivated by the determinism of rules and adaptability of LLMs, we propose a hybrid approach consisting of three modules. We not only write prompts to instruct LLMs to complete tasks, but we also invoke Analytic Rule Interfaces (ARIs) to accomplish tasks. The ARIs are Python code generated by prompting LLMs to generate code. We first construct a knowledge module with three elements including ASTscenario, ASTcomponent and Condition, and prompt LLMs to generate Python code for incorporation into an ARI library for subsequent use. After that, for any syntax-error-free Python code, we invoke ARIs from the ARI library to extract ASTcomponent from the ASTscenario, and then filter out ASTcomponent that does not meet the condition. Finally, we design prompts to instruct LLMs to abstract and idiomatize code, and then invoke ARIs from the ARI library to rewrite non-idiomatic code into the idiomatic code. Next, we conduct a comprehensive evaluation of our approach, RIdiom, and Prompt-LLM on nine established Pythonic idioms in RIdiom. Our approach exhibits superior accuracy, F1-score, and recall, while maintaining precision levels comparable to RIdiom, all of which consistently exceed or come close to 90% for each metric of each idiom. Lastly, we extend our evaluation to encompass four new Pythonic idioms. Our approach consistently outperforms Prompt-LLM, achieving metrics with values consistently exceeding 90% for accuracy, F1-score, precision, and recall.

==> motivation_old.tex <==
% \begin{figure}%[h]
% % \vspace{-0.2cm}
%   \centering
%   % \includegraphics[width=3.4in]{data}
%    \includegraphics[width=4.7in]{data/motivating_example_chain_compare.jpeg}
%   % {data/motivating_example.jpeg}%{data/framework_other_color.png}
%   %{data/framework.png}
% % \setlength{\abovecaptionskip}{-0.1mm}
%     \caption{A motivating example}
%     \label{motiv_example} 
%     % \vspace{-0.3cm}
% \end{figure}

% \begin{figure}%[h]
% % \vspace{-0.2cm}
%   \centering
%   % \includegraphics[width=3.4in]{data}
%    \includegraphics[width=4.7in]{data/motivating_example_list_compre_ridiom.jpeg}
%   % {data/motivating_example.jpeg}%{data/framework_other_color.png}
%   %{data/framework.png}
% % \setlength{\abovecaptionskip}{-0.1mm}
%     \caption{A motivating example that RIdiom cannot find code that can be refactored with list comprehension}
%     \label{motiv_example_ridiom} 
%     % \vspace{-0.3cm}
% \end{figure}
% \begin{figure}%[h]
% % \vspace{-0.2cm}
%   \centering
%   % \includegraphics[width=3.4in]{data}
%    \includegraphics[width=5in]{data/motivating_example_set_compre_llm.jpeg}
%   % {data/motivating_example.jpeg}%{data/framework_other_color.png}
%   %{data/framework.png}
% % \setlength{\abovecaptionskip}{-0.1mm}
%     \caption{A motivating example that directly using LLMs miss code and find wrong code that can be refactored with set comprehension}
%     \label{motiv_example_llm} 
%     % \vspace{-0.3cm}
% \end{figure}
% \begin{figure}%[h]
% % \vspace{-0.2cm}
%   \centering
%   % \includegraphics[width=3.4in]{data}
%    \includegraphics[width=5.4in]{data/motivating_example_star_call.jpeg}
%   % {data/motivating_example.jpeg}%{data/framework_other_color.png}
%   %{data/framework.png}
% % \setlength{\abovecaptionskip}{-0.1mm}
%     \caption{A motivating example}
%     \label{motiv_example_star} 
%     % \vspace{-0.3cm}
% \end{figure}
Although using pythonic idioms can improve the conciseness and performance~\cite{zhang2022making,alexandru2018usage,faster_slower,leelaprute2022does}, refactoring non-idiomatic Python code with pythonic idioms for a given Python code is not easy because of its two challenges. 

% \begin{enumerate}[left=0pt]

\noindent (1) For a given Python code, finding refactorable non-idiomatic code from it is like a needle in a haystack. 
It is challenging to ensure the correctness and completeness of non-idiomatic code detection. 
    % correctly find refactorable non-idiomatic code and 
% make sure no non-idiomatic code is missed.
% the correctness can cause code missing and wrong finding of non-idiomatic code. 
First, the given code may have many number of lines and have various statements and expressions, but the target non-idiomatic code is a small part of the given code. 
For example, the line number of the Python method is 786~\footnote{https://github.com/polakowo/vectorbt/blob/master/vectorbt/signals/factory.py
}, and the refactorable non-idiomatic code of chain-comparison, ``\textsf{cache is None and cache\_func is not None}'' is only one line. 
Second, the given code may have several refactorable non-idiomatic code. 
For example, the \textsf{forward} Python method~\footnote{https://github.com/BachiLi/diffvg/blob/master/pydiffvg/render\_pytorch.py} has more than 10 non-idiomatic code snippets that can be refactored with star-in-func-call, e.g., ``\textsf{diffvg.Vector2f(center[0], center[1])}'' can be refactored into ``\textsf{diffvg.Vector2f(*center[:2])}''.
Finally, the refactorable non-idiomatic code may be logically complex. 
For example, for the first refactorable non-idiomatic code with set-comprehension of Figure~\ref{motiv_example_RIdiom}, the first two if statements of its body have control dependency on the ``\textsf{df.add(y)}'' because of appearance of two continue statements. 
Although the idiomatic code of set-comprehension cannot support continue statement, the non-idiomatic code is refactorable with set-comprehension. 
a[k+1], a[2*k+1];; 
a[-1], a[-2];;
a[`k'], a[`2*k'];;
a[-1], a[0];

    % it is easy to miss it. 
    % shows the refactorable non-idiomatic code that has control dependency or data dependency.
%     And unrelated code appears intermixed with the target code to further increase the difficulty of searching. 
%     For example, the line number of the Python method is 786~\footnote{https://github.com/polakowo/vectorbt/blob/master/vectorbt/signals/factory.py
% }, and the refactorable non-idiomatic code of chain-comparison, ``\textsf{cache is None and cache\_func is not None}'' is only one line. 

\noindent (2) The diversity and complexity of refactorable non-idiomatic code with pythonic idioms makes it challenging to correctly refactor code. 
For example, the first non-idiomatic code of Figure~\ref{motiv_example_RIdiom} shows the refactorable non-idiomatic code that has control dependency or data dependency. 
If we want to refactor it into idiomatic code, we not only need to orderly put ``\textsf{for}'' and ``\textsf{if}'' keywords into set comprehension but also need to do semantic transformation. 
Specifically, we first need to rewrite ``\textsf{z is x}'' and ``\textsf{z not in df}'' as ``\textsf{z is not x}'' and ``\textsf{z in df}'', and then we use the ``\textsf{and}'' to connect the two conditions.
Finally we transform it with set comprehension. 
    % For example, multiple arguments in a function call ``\textsf{mlp\_channels[i], mlp\_channels[i+1]}'', ``\textsf{handles[-2], handles[-1]}'', and ``\textsf{inst.size()[2], inst.size()[3]}'' are both can be refactored with star-in-func-call.
    % Figure~\ref{motiv_example} lists one refactorable non-idiomatic code instance of list-comprehension idiom which exist control dependency.
    % For example, the non-idiomatic code of chain-comparison may have multiple comparison operations: \textsf{if j + k > last\_seen[1] and j + k >= 0 and j + k < len(split\_docs[i]} (the operations are >, >= and <),  \textsf{assert ``http'' in c and c[``http''] == ``http''} (the operations are in and ==), \textsf{if cache is None and cache\_func is not None} (the operations are is and is not) and etc..

% \end{enumerate} 
% To alleviate the two challenges of code refactoring of pythonic idioms, adopting a traditional rules-based approach is not a wise choice. 
% When there are new pythonic idioms, we need to formulate new rules. 
% And the more varied the form of the code, the more code will be lost or be refactored wrongly. 
% For example, state-of-the-art of rules-based tool RIdiom~\cite{zhang2022making} is only limited to nine pythonic idioms, and it wrongly refactors ``\textsf{start is not None and end is not None and start > end}'' into ``\textsf{None is not start is not end > end}'' in Figure~\ref{motiv_example}.
% cannot find the refactorable non-idiomatic code with list-comprehension in Figure~\ref{motiv_example}.
% it finds refactorable non-idiomatic code \textsf{j + k >= 0 and j + k < len(split\_docs[i])} but does not find refactorable non-idiomatic code \textsf{j + k > last\_seen[1] and j + k >= 0} for the chain-comparison idiom. 

% Although large language models (LLMs) has achieved great success on various software engineering tasks~\cite{brown2020language, openai2023gpt4,feng2023prompting,peng2023generative,huang2023ai} by only using natural language prompts,
% directly using LLMs to complete the task is not cost effective. 
% Putting the whole code into LLMs is expensive.
% And it may find wrong non-idiomatic code or miss refactorable non-idiomatic code. 
% For example, directly using LLMs wrongly finds code ``\textsf{start != self.start or end != self.end}'' that cannot be refactored with chain comparison because it does not have the same compare operand and it is also an or boolean operation. 
% And for the found code ``\textsf{start is not None and end is not None and start > end}'', it does not use chain comparison to refactor, but uses truth test to refactor ``\textsf{start is not None}'' into ``\textsf{start}''.
% Figure~\ref{motiv_example} shows such an missed refactorable non-idiomatic code.
% For example, for the chain-comparison, putting the whole code into LLMs, LLMs miss
% non-idiomatic code \textsf{if j + k > last\_seen[1] and j + k >= 0 and j + k < len(split\_docs[i]}, and found non-idiomatic code that cannot refactor with chain-comparison \textsf{objPos[2] >= (heightTarget-tolerance) and reachDist < 0.04} and refactor it into \textsf{heightTarget - tolerance <= objPos[2] < 0.04 + heightTarget - tolerance}. 

% We can see that rules-based approach is too deterministic and directly using LLMs is too blind. 
% So we can make LLMs generate code to complete the deterministic task and then prompt LLMs to complete the challenging refactoring task that using rule-based approach is hard to ensure the completeness of rules.  
% Specifically, non-idiomatic code has deterministic node composition, so
% we can first extract possible refactorable code using code generated by LLMs based on the deterministic node composition.  
% For example, the non-idiomatic code of chain-comparison must have at least two Compare node in a ``and'' boolean operation. 
% For example, chain-comparison is used to refactor ``a op1 b and b op2 c'' into ``a op1 b op2 c''.
% The non-idiomatic code consists of two comparison operations that has the same operand in an and boolean operation. 
% So we can use code generated by LLMs to complete the task. 
% As a result, there are three non-idiomatic code instances ( (e.g., \textsf{start is not None}, \textsf{end is not None}, the same compare operand is \textsf{None}).
% directly use code to extract two comparison operations that has the same operand in the boolean operation. 
% And the code can be generated by LLMs.
% first generate code using LLMs to extract two comparison operations that has the same operand in the boolean operation.
% And then we prompt LLMs do the difficult refactoring task.
% that using rule-based approach is hard to ensure the completeness of rules. 
% For example, we prompt LLMs to reverse the comparison operands of each comparison operation. code with list-comprehension, the non-idiomatic code of Figure~\ref{motiv_example}
% could be found. 
% For example, we can prompt LLMs to reverse comparison operands of two comparison operations to make the same operand is adjacent to \textsf{and}. 
% Specifically, the ``\textsf{start is not None and end is not None}'' is transformed into ``\textsf{start is not None and None is not end}'', and then we can directly replace ``\textsf{None and None}'' with ``\textsf{None}'' to complete the refactoring.
% So \textsf{start is not None and end is not None} is changed to \textsf{start is not None and None is not end}, then we could directly replacing \textsf{None and None} with \textsf{None} to complete refactoring. 
% For example, we prompt LLMs to refactor the code with list-comprehension, the non-idiomatic code of Figure~\ref{motiv_example}
% could be found.% XXXX. star-in-call / chain-comparison/ list comprehension.

\begin{figure}%[h]
% \vspace{-0.2cm}
  \centering
  % \includegraphics[width=3.4in]{data}
   \includegraphics[width=4.4in]{data/motivating_example_RIdiom.png}
  % {data/motivating_example.jpeg}%{data/framework_other_color.png}
  %{data/framework.png}
% \setlength{\abovecaptionskip}{-0.1mm}
    \caption{Motivating examples using RIdiom to refactor non-idiomatic code into idiomatic code with pythonic idioms}
    \label{motiv_example_RIdiom} 
    % \vspace{-0.3cm}
\end{figure}

To alleviate the two challenges of code refactoring of pythonic idioms, adopting a traditional rules-based approach is not a wise choice. 
On the one hand, the diverse and complex form of the non-idiomatic code make non-idiomatic code lost, wrongly find or wrongly refactor. 
State-of-the-art of rules-based tool RIdiom~\cite{zhang2022making} manually formulates detection and refactoring rules for nine pythonic idioms (e.g., set comprehension).
% , it may miss non-idiomatic code or find wrong non-idiomatic code. 
For example, in Figure~\ref{motiv_example_RIdiom}, for the set-comprehension, it can only find for statement whose body has one if or for statement. 
Since the non-idiomatic code has two extra if statements, it misses the non-idiomatic code. 
% and it cannot find code that has data dependencies that can be refactored by the list comprehension idiom (seen in Figure~\ref{motiv_example_ridiom}). 
For another example, for the star-in-func-call, 
RIdiom wrongly think ``\textsf{a[-1], a[9]}'' can be unpacked with a slice object ``\textsf{a[-1:19:10]}''. 
The ``\textsf{a[-1:19:10]}'' actually is an empty list because Python lists grow linearly and are not cyclic, as such slicing does not wrap (from end back to start going forward). 
%https://stackoverflow.com/questions/48776238/python-slice-operator-negative-start-combined-with-positive-stop 
For the last example, for the chain-comparison, 
two comparison operations of the ``\textsf{a != c > d and a > b
}'' code have the common compare operand  ``\textsf{a}''.  
To make ``\textsf{a and a}'' occur in the code, RIdiom first reverses compare operands of ``\textsf{a != c > d}''.
Since RIdiom formulates wrong rules to handle more than two compare operands, ``\textsf{a != c > d}'' is wrongly transformed into ``\textsf{d < c > a}'' which causes the error of the final idiomatic code. 
On the other hand, when there are new pythonic idioms, rule-based approach needs developers to formulate new rules, which is not scalable friendly.

\begin{figure}%[h]
% \vspace{-0.2cm}
  \centering
  % \includegraphics[width=3.4in]{data}
   \includegraphics[width=5.3in]{data/motivating_example_prompt_llm.png}
  % {data/motivating_example.jpeg}%{data/framework_other_color.png}
  %{data/framework.png}
% \setlength{\abovecaptionskip}{-0.1mm}
    \caption{Motivating examples directly using LLM to refactor non-idiomatic code into idiomatic code with pythonic idioms}
    \label{motiv_example_prompt_llm} 
    % \vspace{-0.3cm}
\end{figure}
Although large language models (LLMs) has achieved great success on various software engineering tasks~\cite{brown2020language, openai2023gpt4,feng2023prompting,peng2023generative,huang2023ai} by using natural language prompts, directly using LLMs to complete the task is not cost effective. 
Putting the whole code into LLMs is expensive.
And it may miss non-idiomatic code, find wrong non-idiomatic code or wrongly refactor non-idiomatic code. 
For the first example in Figure~\ref{motiv_example_prompt_llm}, directly using LLMs cannot find true non-idiomatic code that can be refactored with set comprehension, and wrongly finds code ``\textsf{... permissions[...]} = \textsf{in\_roles}'' that can be refactored with dict comprehension instead of set comprehension. 
For the second example in Figure~\ref{motiv_example_prompt_llm}, for two comparison opeations ``\textsf{0 < y\_int < h\_i}'' and ``\textsf{w\_i < 0}'', LLMs wrongly thinks the ``\textsf{h\_i}'' is the common operand and wrongly refactors it into ``\textsf{0 < y\_int < h\_i > w\_i < 0}'', but the correct idiomatic code is ``\textsf{w\_i < 0 < y\_int < h\_i}''.
%可以加xiaoxue ase论文引用


We can see that rules-based approach is too deterministic to find all non-idiomatic code and some code is difficult to complete by manually formulating rules (e.g., the first example of non-idiomatic code that has control dependency in Figure~\ref{motiv_example_RIdiom}).  
And directly using LLMs lacks guidance leading to missing, wrong finding and refactoring errors.  
For example, in Figure~\ref{motiv_example_RIdiom}, the first example of refactorable non-idiomatic code with set comprehension should contain an add function call. 
So we can make LLMs generate code to complete the deterministic task and then prompt LLMs to complete the challenging refactoring task that using rule-based approach is hard to do.  
Specifically, non-idiomatic code has deterministic AST node composition, so
we can first extract possible refactorable code using code generated by LLMs based on the deterministic node composition.  
For example, the non-idiomatic code of set comprehension must be a For node with an add function call. 
And then we prompt LLMs do the difficult refactoring task. 
% For example, we can prompt LLMs to refactor the extracted code with set comprehension. 


% To alleviate the two challenges of code refactoring of pythonic idioms, adopting a traditional rules-based approach is not a wise choice. 
% When there are new pythonic idioms, we need to formulate new rules. 
% And the more varied the form of the code, the more code will be lost or be refactored wrongly. 
% For example, state-of-the-art of rules-based tool RIdiom~\cite{zhang2022making} is only limited to nine pythonic idioms, and it cannot find code that ``\textsf{t\_pair[5], t\_pair[4]}'' that can be refactored with star-in-func-call idiom (seen in Figure~\ref{motiv_example_star}). 


% Although large language models (LLMs) has achieved great success on various software engineering tasks~\cite{brown2020language, openai2023gpt4,feng2023prompting,peng2023generative,huang2023ai} by only using natural language prompts,
% directly using LLMs to complete the task is not cost effective. 
% Putting the whole code into LLMs is expensive.
% And it may find wrong non-idiomatic code or miss refactorable non-idiomatic code. 
% For example, in Figure~\ref{motiv_example_llm}, directly using LLMs misses true refactorable non-idiomatic code with star-in-func-call ``\textsf{t\_pair[5], t\_pair[4]}''.
% And it finds code that cannot be refactored with star-in-func-star and wrongly refactors it, i.e., refactoring ``\textsf{t\_pair[5], t\_pair[4]}'' into ``*t\_pair[5]''.

% We can see that rules-based approach is too deterministic and directly using LLMs is too blind. 
% So we can make LLMs generate code to complete the deterministic task and then prompt LLMs to complete the challenging refactoring task that using rule-based approach is hard to ensure the completeness of rules.  
% Specifically, non-idiomatic code has deterministic node composition, so
% we can first extract possible refactorable code using code generated by LLMs based on the deterministic node composition.  
% For example, the non-idiomatic code of star-in-func-call must be consecutive Subscript node that has the same value. 
% And then we prompt LLMs do the difficult refactoring task. 
% For example, we can prompt LLMs to refactor the extracted code with the slice operator. 
% Then we can directly rewriting it by joining * and the sliced iterable.
